Neural Additive Models for Location Scale and Shape: A Framework for Interpretable Neural Regression Beyond the Mean

Deep neural networks (DNNs) have proven to be highly effective in a variety of tasks, making them the go-to method for problems requiring high-level predictive power. Despite this success, the inner workings of DNNs are often not transparent, making them difficult to interpret or understand. This lack of interpretability has led to increased research on inherently interpretable neural networks in recent years. Models such as Neural Additive Models (NAMs) achieve visual interpretability through the combination of classical statistical methods with DNNs. However, these approaches only concentrate on mean response predictions, leaving out other properties of the response distribution of the underlying data. We propose Neural Additive Models for Location Scale and Shape (NAMLSS), a modelling framework that combines the predictive power of classical deep learning models with the inherent advantages of distributional regression while maintaining the interpretability of additive models. The code is available at the following link: https://github.com/AnFreTh/NAMpy

==> structure/structure_2out.tex <==

 
% Input layer neurons'number
\newcommand{\inputnum}{1} 
 
% Hidden layer neurons'number
\newcommand{\hiddennum}{4}  

% Hidden layer neurons'number
\newcommand{\hiddennumm}{4} 

% dotnumbers
\newcommand{\dotnum}{3} 
 
% Output layer neurons'number
\newcommand{\outputnum}{2} 

\begin{tikzpicture}[scale=0.5]
 
% Input Layer
\foreach \i in {1,...,\inputnum}
{
    \node[circle, 
        minimum size = 4mm,
        fill=white!30!black] (Input-\i) at (0,0.5) {};
}


 \foreach \i in {1}
{
        \draw[->, shorten <=1pt] (9.5, -0.2) -- ++(+2.5,0.0)
        node[circle, 
        minimum size = 1mm,
        fill=green!10!white, right]{$\hat{\theta}^{(1)}$};
        \node[] at (10.75,0.5) {$h^{(1)}$};
}

 \foreach \i in {1}
{
        \draw[->, shorten <=1pt] (9.5, -4.2) -- ++(+2.5,0.0)
        node[circle, 
        minimum size = 1mm,
        fill=green!10!white, right]{$\hat{\theta}^{(2)}$};
        \node[] at (10.75, -3.5) {$h^{(2)}$};
}


% draw rectangles around mlps
\node[rectangle,
    draw = blue,
    minimum width = 3.5cm, 
    minimum height = 2.1cm] (r) at (1,0.5) {};
    
\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.2,-1.5) {};

\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.4,-2.5) {};


\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.6,-3.5) {};

\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.8,-4.5) {};
    
\node[rectangle,
    draw = blue,
    minimum width = 3.5cm, 
    minimum height = 2.1cm] (r) at (1,-5.5) {};


 
% Hidden Layer
\foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        minimum size = 4mm,
        fill=blue!20!white,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-\i) at (1,-\i) {};
}

\foreach \i in {1, ..., \dotnum}
{
    \node[yshift=(\dotnum-\inputnum)*5 mm](Dots-\i) at (2,-\i){\vdots};
}

% Hidden Layer
\foreach \i in {1,...,\hiddennumm}
{
    \node[circle, 
        minimum size = 4mm,
        fill=blue!20!white,
        yshift=(\hiddennumm-\inputnum)*5 mm
    ] (Hidden1-\i) at (3,-\i) {};
}


% Output Layer
\foreach \i in {1,...,\outputnum}
{
    \node[circle, 
        minimum size = 3mm,
        fill=gray!50,
        yshift=(\outputnum-\inputnum)*5 mm
    ] (Output-\i) at (5,-1*\i+1) {$z_\i$};
}

 
% Connect neurons In-Hidden
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Input-\i) -- (Hidden-\j);   
    }
}
 
% Connect neurons Hidden-dots
\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\dotnum}
    {
        \draw[-,path fading=east] (Hidden-\i) -- (Dots-\j);
    }
}

% Connect neurons dots hidden
\foreach \i in {1,...,\dotnum}
{
    \foreach \j in {1,...,\hiddennumm}
    {
        \draw[-,path fading=west] (Dots-\i) -- (Hidden1-\j);
    }
}

% Connect neurons Hidden-Output
\foreach \i in {1,...,\hiddennumm}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden1-\i) -- (Output-\j);
    }
}
 
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Input-\i) -- ++(-1,0)
        node[left]{$x_{1}$};
}
 
% Outputs

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% add output in the middle)

 \foreach \i in {1,...,2}
{
    \node[circle, 
        minimum size = 1mm,
        fill=yellow!50, yshift=(\dotnum-\inputnum-3)*5 mm](SUM-\i) at (8.5,-3.67*\i+4){$\sum_{j=1}^{J}$};
}


        



%%%%%%%%%%%%%%%%%%%%%%% add dots in the middle %%%%%%%%%%%%%%%%%%%
 
 \foreach \i in {1, ..., 2}
{
    \node[yshift=(\dotnum-\inputnum-3)*5 mm](Dotsm-\i) at (2,-\i){\vdots};
}

%%%%%%%%%%%%%%%%%%%%%%% connect dots in the middle %%%%%%%%%%%%%%%%%%%%%%%%

\foreach \i in {1,...,2}
{
        \draw[-, shorten >=1pt, path fading=west] (Dotsm-\i) -- (SUM-\i);   
}


\foreach \i in {1,...,1}
{            
    \draw[-, shorten <=2pt] (Output-\i) -- ++(2.5, -1)
        node[right]{};
}

\foreach \i in {2,...,2}
{            
    \draw[-, shorten <=2pt] (Output-\i) -- ++(2.5, -4)
        node[right]{};
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%second one %%%%%%%%%%%%%%%%%
 
% Input Layer
\foreach \i in {1,...,\inputnum}
{
    \node[circle, 
        minimum size = 4mm,
        fill=white!30!black] (Inputk-\i) at (0,-\i-4.5) {};
}
 
% Hidden Layer
\foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        minimum size = 4mm,
        fill=blue!20!white,
        yshift=(\hiddennum-\inputnum-3)*5 mm
    ] (Hiddenk-\i) at (1,-\i-3) {};
}

% dots
\foreach \i in {1, ..., \dotnum}
{
    \node[yshift=(\dotnum-\inputnum-2.5)*5 mm](Dotsk-\i) at (2,-\i-2.5){\vdots};
}

% Hidden Layer
\foreach \i in {1,...,\hiddennumm}
{
    \node[circle, 
        minimum size = 4mm,
        fill=blue!20!white,
        yshift=(\hiddennumm-\inputnum-3)*5 mm
    ] (Hidden1k-\i) at (3,-\i -3) {};
}


% Output Layer
\foreach \i in {1,...,2}
{
    \node[circle, 
        minimum size = 3mm,
        fill=gray!50,
        yshift=(\outputnum-\inputnum-)*5  mm
    ] (Outputk-\i) at (5,-\i -5) {$z_\i$};
}
 
% Connect neurons In-Hidden
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Inputk-\i) -- (Hiddenk-\j);   
    }
}
 
% Connect neurons Hidden-dots
\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\dotnum}
    {
        \draw[-,path fading=east] (Hiddenk-\i) -- (Dotsk-\j);
    }
}

% Connect neurons dots hidden
\foreach \i in {1,...,\dotnum}
{
    \foreach \j in {1,...,\hiddennumm}
    {
        \draw[-,path fading=west] (Dotsk-\i) -- (Hidden1k-\j);
    }
}

% Connect neurons Hidden-Output
\foreach \i in {1,...,\hiddennumm}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden1k-\i) -- (Outputk-\j);
    }
}
 
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Inputk-\i) -- ++(-1,0)
        node[left]{$x_{J}$};
}
 
% Outputs
\foreach \i in {1,...,1}
{            
    \draw[-, shorten <=2pt] (Outputk-\i) -- ++(2.5, 4)
        node[right]{};
}

\foreach \i in {2,...,2}
{            
    \draw[-, shorten <=2pt] (Outputk-\i) -- ++(2.5, 1)
        node[right]{};
}


\end{tikzpicture}



==> structure/structure_tikz_loc.tex <==

 
% Input layer neurons'number
\newcommand{\inputnum}{1} 
 
% Hidden layer neurons'number
\newcommand{\hiddennum}{4}  

% Hidden layer neurons'number
\newcommand{\hiddennumm}{4} 

% dotnumbers
\newcommand{\dotnum}{3} 
 
% Output layer neurons'number
\newcommand{\outputnum}{1} 

\begin{tikzpicture}[scale=0.5]
 
% Input Layer
\foreach \i in {1,...,\inputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=white!30!black] (Input-\i) at (0,0.5) {};
}

\draw [decorate,decoration={brace,amplitude=20pt, mirror},xshift=4pt,yshift=0pt]
(-3, 2.5) -- (-3, -1.5) node [black,midway,xshift=-1cm]
{$f_{1}^{(1)}$};



\draw [decorate,decoration={brace,amplitude=20pt, mirror},xshift=4pt,yshift=0pt]
(-3, -3.5) -- (-3, -7.5) node [black,midway,xshift=-1cm]
{$f_{J}^{(1)}$};


% draw rectangles around mlps
\node[rectangle,
    draw = blue,
    minimum width = 3.5cm, 
    minimum height = 2.1cm] (r) at (1,0.5) {};
    
\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.2,-1.5) {};

\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.4,-2.5) {};


\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.6,-3.5) {};

\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.8,-4.5) {};
    
\node[rectangle,
    draw = blue,
    minimum width = 3.5cm, 
    minimum height = 2.1cm] (r) at (1,-5.5) {};


 
% Hidden Layer
\foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-\i) at (1,-\i) {};
}

\foreach \i in {1, ..., \dotnum}
{
    \node[yshift=(\dotnum-\inputnum)*5 mm](Dots-\i) at (2,-\i){\vdots};
}

% Hidden Layer
\foreach \i in {1,...,\hiddennumm}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennumm-\inputnum)*5 mm
    ] (Hidden1-\i) at (3,-\i) {};
}


% Output Layer
\foreach \i in {1,...,\outputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=gray!50,
        yshift=(\outputnum-\inputnum)*5 mm
    ] (Output-\i) at (4,0.5) {};
}
 
% Connect neurons In-Hidden
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Input-\i) -- (Hidden-\j);   
    }
}
 
% Connect neurons Hidden-dots
\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\dotnum}
    {
        \draw[-,path fading=east] (Hidden-\i) -- (Dots-\j);
    }
}

% Connect neurons dots hidden
\foreach \i in {1,...,\dotnum}
{
    \foreach \j in {1,...,\hiddennumm}
    {
        \draw[-,path fading=west] (Dots-\i) -- (Hidden1-\j);
    }
}

% Connect neurons Hidden-Output
\foreach \i in {1,...,\hiddennumm}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden1-\i) -- (Output-\j);
    }
}
 
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Input-\i) -- ++(-1,0)
        node[left]{$x_{1}$};
}
 
% Outputs

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% add output in the middle)

 \foreach \i in {1}
{
    \node[circle, 
        minimum size = 1mm,
        fill=yellow!50, yshift=(\dotnum-\inputnum-3)*5 mm](SUM-\i) at (5.5,-\i-0.3){$\sum_{j=1}^{J}$};
}

 \foreach \i in {1}
{
        \draw[->, shorten <=1pt] (SUM-\i) -- ++(+1.5,0)
        node[circle, 
        minimum size = 1mm,
        fill=green!10!white, right]{$\hat{\theta}^{(1)}$};
        \node[] at (6.75,-1.8) {$h^{(1)}$};
}

        



%%%%%%%%%%%%%%%%%%%%%%% add dots in the middle %%%%%%%%%%%%%%%%%%%
 
 \foreach \i in {1, ..., 2}
{
    \node[yshift=(\dotnum-\inputnum-3)*5 mm](Dotsm-\i) at (2,-\i){\vdots};
}

%%%%%%%%%%%%%%%%%%%%%%% connect dots in the middle %%%%%%%%%%%%%%%%%%%%%%%%

\foreach \i in {1,...,2}
{
        \draw[-, shorten >=1pt, path fading=west] (Dotsm-\i) -- (SUM-1);   
}


\foreach \i in {1,...,\outputnum}
{            
    \draw[-, shorten <=2pt] (Output-\i) -- ++(1.5, -2)
        node[right]{};
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%second one %%%%%%%%%%%%%%%%%
 
% Input Layer
\foreach \i in {1,...,\inputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=white!30!black] (Inputk-\i) at (0,-\i-4.5) {};
}
 
% Hidden Layer
\foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennum-\inputnum-3)*5 mm
    ] (Hiddenk-\i) at (1,-\i-3) {};
}

% dots
\foreach \i in {1, ..., \dotnum}
{
    \node[yshift=(\dotnum-\inputnum-2.5)*5 mm](Dotsk-\i) at (2,-\i-2.5){\vdots};
}

% Hidden Layer
\foreach \i in {1,...,\hiddennumm}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennumm-\inputnum-3)*5 mm
    ] (Hidden1k-\i) at (3,-\i -3) {};
}


% Output Layer
\foreach \i in {1,...,\outputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=gray!50,
        yshift=(\outputnum-\inputnum-1.5)*5  mm
    ] (Outputk-\i) at (4,-\i -3) {};
}
 
% Connect neurons In-Hidden
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Inputk-\i) -- (Hiddenk-\j);   
    }
}
 
% Connect neurons Hidden-dots
\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\dotnum}
    {
        \draw[-,path fading=east] (Hiddenk-\i) -- (Dotsk-\j);
    }
}

% Connect neurons dots hidden
\foreach \i in {1,...,\dotnum}
{
    \foreach \j in {1,...,\hiddennumm}
    {
        \draw[-,path fading=west] (Dotsk-\i) -- (Hidden1k-\j);
    }
}

% Connect neurons Hidden-Output
\foreach \i in {1,...,\hiddennumm}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden1k-\i) -- (Outputk-\j);
    }
}
 
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Inputk-\i) -- ++(-1,0)
        node[left]{$x_{J}$};
}
 
% Outputs
\foreach \i in {1,...,\outputnum}
{            
    \draw[-, shorten <=2pt] (Outputk-\i) -- ++(1.5, 2.4)
        node[right]{};
}


\end{tikzpicture}



==> structure/structure_tikz_scale.tex <==


\begin{tikzpicture}[scale=0.5]


% draw rectangles around mlps
\node[rectangle,
    draw = blue,
    minimum width = 3.5cm, 
    minimum height = 2.1cm] (r) at (1,0.5) {};
    
\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.2,-1.5) {};

\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.4,-2.5) {};


\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.6,-3.5) {};

\node[rectangle,
    draw = blue!20,
    minimum width = 3.5cm, 
    minimum height = 0.6cm] (r) at (1.8,-4.5) {};
    
\node[rectangle,
    draw = blue,
    minimum width = 3.5cm, 
    minimum height = 2.1cm] (r) at (1,-5.5) {};
 
% Input Layer
\foreach \i in {1,...,\inputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=white!30!black] (Input-\i) at (0,0.5) {};
}
 
% Hidden Layer
\foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-\i) at (1,-\i) {};
}

\foreach \i in {1, ..., \dotnum}
{
    \node[yshift=(\dotnum-\inputnum)*5 mm](Dots-\i) at (2,-\i){\vdots};
}

% Hidden Layer
\foreach \i in {1,...,\hiddennumm}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennumm-\inputnum)*5 mm
    ] (Hidden1-\i) at (3,-\i) {};
}


% Output Layer
\foreach \i in {1,...,\outputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=gray!50,
        yshift=(\outputnum-\inputnum)*5 mm
    ] (Output-\i) at (4,0.5) {};
}
 
% Connect neurons In-Hidden
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Input-\i) -- (Hidden-\j);   
    }
}
 
% Connect neurons Hidden-dots
\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\dotnum}
    {
        \draw[-,path fading=east] (Hidden-\i) -- (Dots-\j);
    }
}

% Connect neurons dots hidden
\foreach \i in {1,...,\dotnum}
{
    \foreach \j in {1,...,\hiddennumm}
    {
        \draw[-,path fading=west] (Dots-\i) -- (Hidden1-\j);
    }
}

% Connect neurons Hidden-Output
\foreach \i in {1,...,\hiddennumm}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden1-\i) -- (Output-\j);
    }
}
 
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Input-\i) -- ++(-1,0)
        node[left]{$x_{1}$};
}
 
% Outputs

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% add output in the middle)

 \foreach \i in {1}
{
    \node[circle, 
        minimum size = 1mm,
        fill=yellow!50, yshift=(\dotnum-\inputnum-3)*5 mm](SUM-\i) at (5.5,-\i-0.3){$\sum_{j=1}^{J}$};
}

 \foreach \i in {1}
{
        \draw[->, shorten <=1pt] (SUM-\i) -- ++(+1.5,0)
        node[circle, 
        minimum size = 1mm,
        fill=green!10!white, right]{$\hat{\theta}^{(2)}$};
        \node[] at (6.75,-1.8) {$h^{(2)}$};
}



        



%%%%%%%%%%%%%%%%%%%%%%% add dots in the middle %%%%%%%%%%%%%%%%%%%
 
 \foreach \i in {1, ..., 2}
{
    \node[yshift=(\dotnum-\inputnum-3)*5 mm](Dotsm-\i) at (2,-\i){\vdots};
}

%%%%%%%%%%%%%%%%%%%%%%% connect dots in the middle %%%%%%%%%%%%%%%%%%%%%%%%

\foreach \i in {1,...,2}
{
        \draw[-, shorten >=1pt, path fading=west] (Dotsm-\i) -- (SUM-1);   
}


\foreach \i in {1,...,\outputnum}
{            
    \draw[-, shorten <=2pt] (Output-\i) -- ++(1.5, -2)
        node[right]{};
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%second one %%%%%%%%%%%%%%%%%
 
% Input Layer
\foreach \i in {1,...,\inputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=white!30!black] (Inputk-\i) at (0,-\i-4.5) {};
}
 
% Hidden Layer
\foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennum-\inputnum-3)*5 mm
    ] (Hiddenk-\i) at (1,-\i-3) {};
}

% dots
\foreach \i in {1, ..., \dotnum}
{
    \node[yshift=(\dotnum-\inputnum-2.5)*5 mm](Dotsk-\i) at (2,-\i-2.5){\vdots};
}


\draw [decorate,decoration={brace,amplitude=20pt, mirror},xshift=4pt,yshift=0pt]
(-3, 2.5) -- (-3, -1.5) node [black,midway,xshift=-1cm]
{$f_{1}^{(2)}$};

\draw [decorate,decoration={brace,amplitude=20pt, mirror},xshift=4pt,yshift=0pt]
(-3, -3.5) -- (-3, -7.5) node [black,midway,xshift=-1cm]
{$f_{J}^{(2)}$};







% Hidden Layer
\foreach \i in {1,...,\hiddennumm}
{
    \node[circle, 
        minimum size = 2mm,
        fill=blue!20!white,
        yshift=(\hiddennumm-\inputnum-3)*5 mm
    ] (Hidden1k-\i) at (3,-\i -3) {};
}


% Output Layer
\foreach \i in {1,...,\outputnum}
{
    \node[circle, 
        minimum size = 2mm,
        fill=gray!50,
        yshift=(\outputnum-\inputnum-1.5)*5  mm
    ] (Outputk-\i) at (4,-\i -3) {};
}
 
% Connect neurons In-Hidden
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Inputk-\i) -- (Hiddenk-\j);   
    }
}
 
% Connect neurons Hidden-dots
\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\dotnum}
    {
        \draw[-,path fading=east] (Hiddenk-\i) -- (Dotsk-\j);
    }
}

% Connect neurons dots hidden
\foreach \i in {1,...,\dotnum}
{
    \foreach \j in {1,...,\hiddennumm}
    {
        \draw[-,path fading=west] (Dotsk-\i) -- (Hidden1k-\j);
    }
}

% Connect neurons Hidden-Output
\foreach \i in {1,...,\hiddennumm}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden1k-\i) -- (Outputk-\j);
    }
}
 
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Inputk-\i) -- ++(-1,0)
        node[left]{$x_{J}$};
}
 
% Outputs
\foreach \i in {1,...,\outputnum}
{            
    \draw[-, shorten <=2pt] (Outputk-\i) -- ++(1.5, 2.4)
        node[right]{};
}


\end{tikzpicture}


